Higher Codimension Cycles on the Hilbert Scheme of Three Points on the Projective Plane

In this paper, we study the higher codimensional cycle structure of the Hilbert scheme of three points in the projective plane. In particular, we compute all Chern (and Segre) classes of all tautological bundles on it and compute the nef (effective) cones of cycles in codimensions 2 and 3 (dimensions 2 and 3).

==> locus_C_1.tex <==
\begin{tikzpicture}[framed]
	\def\ptsize{2.0pt}
	
\def\width{2}
\def\height{2}

\draw (\width,\height) circle (0);
\draw (0,0) circle (0);
	
\def\qx{1.5} \def\qy{1.5}
	
\coordinate (Q1) at ($(.5,.25)!.55!(1.75,1.75)$);
\coordinate (Q1`) at ($(Q1) - (.4,-.25)$);


\draw[thick,dashed,->] (Q1) -- (Q1`);

\node[above] at (Q1`) {$3$};		

\fill (Q1) circle (\ptsize);

\end{tikzpicture}

